Popular Knowledge Propagates More Errors in LLM Knowledge Updating

Updating a language model's knowledge through fine-tuning is essential for keeping its outputs current, yet can also induce factual forgetting and new hallucinations. Prior work shows that long-tail knowledge is harder to acquire and newly memorized long-tail facts are difficult to retain during later fine-tuning. We study a complementary question: among facts that a model has encoded correctly, which are most vulnerable to collateral corruption during other updates? To investigate this question under a realistic factual distribution, we construct a large-scale graph FACTPROP of verified Wikipedia facts by linking triples that share head or tail entities, thereby preserving connections among factual knowledge. We fine-tune models on factual statements and measure correct-to-incorrect facts after each update. Our results reveal a pattern distinct from prior findings on long-tail vulnerability during acquisition and retention: among facts that models already answer correctly, those associated with highly connected entities are more likely to be corrupted by neighboring updates, and updates to such facts propagate errors more broadly. Structural popularity therefore predicts both vulnerability and downstream damage. Inspired by this finding, we propose Popularity-based Anchoring (PopAnchor), a lightweight rehearsal strategy that preserves a small set of popular facts and reduces forgetting.

==> contents/ack.tex <==
\section*{Acknowledgments}


==> tables/delta_margin_per_model.tex <==
\begin{table}[t]
\centering
\small
\caption{\textbf{Hub-neighbor margin collapse is consistent across all four evaluated model families.} Mean correct-token margin change $\Delta\mathrm{Margin} = \mathrm{Margin}_{\text{post}} - \mathrm{Margin}_{\text{pre}}$, pooled over $d{=}1$ to $d{=}5$ on the Mask-B subset (pre-update-correct facts; see Section~\ref{sec:setup}). More negative $=$ deeper confidence collapse. The Hub-neighbor column suffers the deepest drop in \textbf{4/4} models (Hub--Tail gap shown in the last column). The signal also persists on the heavily instruction-tuned Gemma-4-E4B-it, where output-level flip behaviour is otherwise heavily suppressed.}
\label{tab:delta_margin_per_model}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lrrrr}
\toprule
\textbf{Model} & \textbf{Hub} & \textbf{Mid} & \textbf{Tail} & \textbf{Hub $-$ Tail} \\
\midrule
Qwen3.5-2B       & $\mathbf{-0.90}$ \tiny{(n{=}8{,}026)}  & $+0.05$ \tiny{(n{=}2{,}901)} & $-0.25$ \tiny{(n{=}199)} & $\mathbf{-0.65}$ \\
Qwen3.5-9B       & $\mathbf{-2.18}$ \tiny{(n{=}10{,}956)} & $-1.80$ \tiny{(n{=}5{,}253)} & $-1.64$ \tiny{(n{=}322)} & $\mathbf{-0.55}$ \\
Gemma-4-E4B-it   & $\mathbf{-0.33}$ \tiny{(n{=}8{,}791)}  & $+0.09$ \tiny{(n{=}2{,}753)} & $+0.48$ \tiny{(n{=}179)} & $\mathbf{-0.81}$ \\
Gemma-4-31B-it   & $\mathbf{-6.65}$ \tiny{(n{=}11{,}703)} & $-5.12$ \tiny{(n{=}5{,}672)} & $-3.79$ \tiny{(n{=}356)} & $\mathbf{-2.86}$ \\
\midrule
\textbf{Hub $>$ Tail collapse} & \multicolumn{4}{c}{\textbf{4 / 4 models}} \\
\bottomrule
\end{tabular}%
}
\end{table}


==> tables/transition_across_graph.tex <==
% === LaTeX Table Generator Output ===
% Requires \usepackage{booktabs} and \usepackage{multirow} in your preamble

% Table 1: Detailed Breakdown of Error Dynamics and Confidence Shifts
\begin{table*}[t]
\centering
\small
\begin{tabular}{llcccccc}
\toprule
Distance & Transition Type & Count & Ratio (\%) & Pre Conf. & Post Conf. & Conf. $\Delta$ \\
\midrule
\multirow{3}{*}{d0} 
& W $\to$ W (Same) & 0 & 0.0 & 0.000 & 0.000 & +0.000 \\
& W $\to$ W (Diff) & 4 & 40.0 & 0.944 & 0.944 & +0.000 \\
& C $\to$ W (Flip) & 3 & 30.0 & 0.926 & 1.000 & +0.074 \\
\cmidrule(lr){1-7}
\multirow{3}{*}{d1} 
& W $\to$ W (Same) & 26 & 1.4 & 0.689 & 0.885 & \textbf{+0.196} \\
& W $\to$ W (Diff) & 212 & 11.6 & 0.878 & 0.919 & +0.041 \\
& C $\to$ W (Flip) & 41 & 2.2 & 0.762 & 0.862 & +0.100 \\
\cmidrule(lr){1-7}
\multirow{3}{*}{d2} 
& W $\to$ W (Same) & 206 & 3.0 & 0.727 & 0.883 & \textbf{+0.157} \\
& W $\to$ W (Diff) & 1604 & 23.6 & 0.807 & 0.906 & +0.099 \\
& C $\to$ W (Flip) & 749 & 11.0 & 0.620 & 0.919 & \textbf{+0.299} \\
\cmidrule(lr){1-7}
\multirow{3}{*}{d3} 
& W $\to$ W (Same) & 290 & 3.4 & 0.822 & 0.890 & +0.068 \\
& W $\to$ W (Diff) & 2473 & 29.0 & 0.738 & 0.898 & \textbf{+0.160} \\
& C $\to$ W (Flip) & 989 & 11.6 & 0.703 & 0.884 & \textbf{+0.181} \\
\cmidrule(lr){1-7}
\multirow{3}{*}{d4} 
& W $\to$ W (Same) & 402 & 3.5 & 0.823 & 0.901 & +0.078 \\
& W $\to$ W (Diff) & 3130 & 27.0 & 0.787 & 0.892 & +0.105 \\
& C $\to$ W (Flip) & 1516 & 13.1 & 0.671 & 0.888 & \textbf{+0.217} \\
\cmidrule(lr){1-7}
\multirow{3}{*}{d5} 
& W $\to$ W (Same) & 718 & 3.8 & 0.820 & 0.893 & +0.074 \\
& W $\to$ W (Diff) & 4649 & 24.9 & 0.732 & 0.901 & \textbf{+0.169} \\
& C $\to$ W (Flip) & 2089 & 11.2 & 0.639 & 0.892 & \textbf{+0.253} \\
\bottomrule
\end{tabular}
\caption{\textbf{Fine-grained breakdown of knowledge transitions across graph distances (Llama-2 paired audit).} \textbf{W $\to$ W (Same)}: persistent errors with identical answers before and after the update. \textbf{W $\to$ W (Diff)}: errors that shifted to a new incorrect answer. \textbf{C $\to$ W (Flip)}: pre-update-correct facts corrupted into errors. The confidence increases in the C $\to$ W cells at $d{=}2$, $d{=}4$, and $d{=}5$ are retained as preliminary evidence from this single-model cohort.}
\label{tab:transition_confidence}
\end{table*}

